On the Partial-Wave Analysis of Mesonic Resonances Decaying to Multiparticle Final States Produced by Polarized Photons

Meson spectroscopy is going through a revival with the advent of high statistics experiments and new advances in the theoretical predictions. The Constituent Quark Model (CQM) is finally being expanded considering more basic principles of field theory and using discrete calculations of Quantum Chromodynamics (lattice QCD). These new calculations are approaching predictive power for the spectrum of hadronic resonances and decay modes. It will be the task of the new experiments to extract the meson spectrum from the data and compare with those predictions. The goal of this report is to describe one particular technique for extracting resonance information from multiparticle final states. The technique described here, partial wave analysis based on the helicity formalism, has been used at Brookhaven National Laboratory (BNL) using pion beams, and Jefferson Laboratory (JLab) using photon beams. In particular this report broadens this technique to include production experiments using linearly polarized real photons or quasi-real photons. This article is of a didactical nature. We describe the process of analysis, detailing assumptions and formalisms, and is directed towards people interested in starting partial wave analysis.

==> SpinDen/partialWaves.tex <==
\subsection{Partial Waves}

Let's put all together now in the expression for the intensity, $I(\tau)$. Let's recall from (\ref{eqn:totall}) that:

\begin{equation}  I(\tau) = \sum_{k,\epsilon,\epsilon'}  \sum_{b,b'} \  {^{\epsilon}V^{k}_{b}}\  {^{\epsilon}A_{b}(\tau)}  { ^{\epsilon\epsilon'}}\rho_{b,b'} {^{\epsilon'}V^{k*}_{b'}}\  {^{\epsilon'}A^{*}_{b'}(\tau)} \end{equation} 

We have organized the indexes such that $k,\epsilon$ are the external or non-interfering indexes. the index $"b"$ contains the characterization of each partial wave (intermediate states) and $\tau$ the angular definition of the final states.

\begin{equation} b=\begin{Bmatrix}I^{G}J^{PC}ML[w_{0},\Gamma_{0}]s\end{Bmatrix} \end{equation}  

where these numbers are:\\

I : isospin of the resonance\\

G: G-parity of the resonance\\

J: total spin of the resonance\\

P: parity of the resonance\\

C: Charge conjugation of the resonance\\

M: spin projection of the resonance about the beam axis (z-direction)\\

L: is the orbital angular momentum between the isobar and the bachelor particle\\

${[w_{0},\Gamma_{0}]}$  the central mass and width of the isobar particle\\

s: the angular momentum between the two daughters of the isobar (spin of isobar)\\

Some of those are related:

\begin{equation}  P=(-1)^{L+1} \end{equation} 
\begin{equation}  C=(-1)^{L+S} \end{equation} 
\begin{equation}  G=(-1)^{L+S+I} \end{equation} 

\begin{equation}  \tau=\begin{Bmatrix}\Omega_{GJ},\Omega_{h},w\end{Bmatrix} \end{equation} 

For our simple two body decay, we have to independent quantum numbers of the decaying particle $I$ and $,J$, and therefore $N_{i}=(2J+1)$ possible states. If the final decay particles have spins $S_{1}$ and $S_{2}$, we will have $N_{f}=(2S_{1}+1)(2S_{2}+1)$ number of final states. The decay matrix connecting the initial and final states will be of dimensions $N_{i}xN_{f}$. 

For each wave (b) we can calculate the decay amplitudes directly from the formulas given in section  3.2. The photon spin density matrix, $^{\epsilon}\rho_{\gamma}$ is calculated with the formulas discussed in section 4. The $^{\epsilon}V_{b}^{k}$ are the parameters of the model (equivalent to $\overrightarrow{a}$ in section 2. Therefore,  for each wave, we will have $k \times 2$ parameters in our model. The factor of two appears because the Vs are complex numbers.

To figure out the number of waves to include in the analysis is a dedicated and reaction dependent decision. We will give some general concepts.

There some relations between the quantum numbers of the resonance and the final states that limited the number of possible waves to include in the set.
Writing:

\begin{equation}   \langle \epsilon,b| ^{\epsilon\epsilon'}\rho_{\gamma} |\epsilon',b'\rangle= \begin{pmatrix}\rho_{11} & \rho_{1-1} \\ \rho_{-11} & \rho_{-1-1}\end{pmatrix} = {\raise0.7ex\hbox{$ 1 $}\!\mathord{\left/{\vphantom{1 2}}\right.\kern-\nulldelimiterspace}\!\lower0.7ex\hbox{$ 2 $}} \left(\begin{array}{cc} {1+P\cos 2\alpha } & {iP\sin 2\alpha } \\ {-iP\sin 2\alpha } & {1-P\cos 2\alpha } \end{array}\right) \end{equation} 

we have


\begin{equation}
 I(\tau)=\sum_{k} \begin{Bmatrix}  \sum_{b,b'}  \begin{pmatrix} {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)\rho_{11}  {^{1}}V_{b'}^{k *}\  {^{1}A^{*}_{b'}(\tau)} + {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)\rho_{1-1}  {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)} \\
 +{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)\rho_{-11}  {^{1}}V_{b'}^{k *}\  {^{1}A^{*}_{b'}(\tau)}+{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)\rho_{-1-1}  {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)}\end{pmatrix} \end{Bmatrix}
 \end{equation}
 
 or
 
 \begin{equation}
 I(\tau)=\sum_{k}  \begin{pmatrix} \rho_{11} \sum_{b,b'} {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)  {^{1}}V_{b'}^{k *}\  {^{1}A^{*}_{b'}(\tau)} + \rho_{1-1} \sum_{b,b'}  {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau) {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)} \\
 +\rho_{-11}\sum_{b,b'}  {^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)  {^{1}}V_{b'}^{k *}\  {^{1}A^{*}_{b'}(\tau)}+\rho_{-1-1} \sum_{b,b'} {^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)  {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)}\end{pmatrix}
 \end{equation}
 
 or, taking the 1/2 outside the $\rho$'s
 
 \begin{equation}
 I(\tau)= \frac{1}{2} \sum_{k}  \begin{pmatrix} \rho_{11} \sum_{b}| {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)|^{2} + \rho_{1-1} \sum_{b,b'}  {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau) {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)} \\
 +\rho_{-11}\sum_{b,b'}  {^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)  {^{1}}V_{b'}^{k *}\  {^{1}A^{*}_{b'}(\tau)}+\rho_{-1-1} \sum_{b} |{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)|^{2} \end{pmatrix}
 \end{equation} 

let's call $\rho_{nd}=iPsin2\alpha=\rho_{1-1}=-\rho_{-11}$ (non-diagonal elements)

then

\begin{equation}
 I(\tau)= \frac{1}{2} \sum_{k}  \begin{pmatrix} \rho_{11} \sum_{b}| {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)|^{2} + \rho_{nd} \sum_{b,b'}[  {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau) {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)} \\
 -{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)  {^{1}}V_{b'}^{k *}\  {^{1}A^{*}_{b'}(\tau)}]+\rho_{-1-1} \sum_{b} |{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)|^{2} \end{pmatrix}
 \end{equation} 
 
 calling $C_{bb'}={^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau) {^{-1}}V_{b'}^{k *}\  {^{-1}A^{*}_{b'}(\tau)}$ we have
 
  \begin{equation}
 I(\tau)= \frac{1}{2} \sum_{k}  \begin{pmatrix} \rho_{11} \sum_{b}| {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)|^{2} + \rho_{nd} \sum_{b,b'}[  C_{bb'} -C^{*}_{bb'}]+\rho_{-1-1} \sum_{b} |{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)|^{2} \end{pmatrix}
 \end{equation} 
 
 and since $C_{bb'}-C^{*}_{bb'}=i \times 2 \times Im(C_{bb'})$
 
 \begin{equation}
 I(\tau)= \frac{1}{2} \sum_{k}  \begin{pmatrix} \rho_{11} \sum_{b}| {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)|^{2} + 2i\rho_{nd}\sum_{b,b'} Im(C_{bb'})+\rho_{-1-1} \sum_{b} |{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)|^{2} \end{pmatrix}
 \end{equation}   
 
 This show that the non-diagonal elements of the photon spin density matrix in the reflectivity basis ($\rho_{nd}$) must be imaginary to make the intensity real as it is the case.

Substituting back the values of $\rho$'s:

\begin{equation}
 I(\tau)= \frac{1}{2} \sum_{k}  [ (1+Pcos2\alpha) \sum_{b}| {^{1}}V_{b}^{k}\  {^{1}}A_{b}(\tau)|^{2} - 2Psin2\alpha \sum_{b,b'} Im(C_{bb'})+(1-Pcos2\alpha)\sum_{b} |{^{-1}}V_{b}^{k}\  {^{-1}}A_{b}(\tau)|^{2} ]
 \end{equation}   


 

